Leveraging LLMs for Dialogue Quality Measurement

In task-oriented conversational AI evaluation, unsupervised methods poorly correlate with human judgments, and supervised approaches lack generalization. Recent advances in large language models (LLMs) show robust zeroshot and few-shot capabilities across NLP tasks. This paper explores using LLMs for automated dialogue quality evaluation, experimenting with various configurations on public and proprietary datasets. Manipulating factors such as model size, in-context examples, and selection techniques, we examine "chain-of-thought" (CoT) reasoning and label extraction procedures. Our results show that (1) larger models yield more accurate dialogue labels; (2) algorithmic selection of in-context examples outperforms random selection; (3) CoT reasoning where an LLM is asked to provide justifications before outputting final labels improves performance; and (4) fine-tuned LLMs outperform out-of-the-box ones. Our results indicate that LLMs that are suitably fine-tuned and have sufficient reasoning capabilities can be leveraged for automated dialogue evaluation.

==> tex/_clutter/Experiment_results-also-old.tex <==
\section{Results}
\label{sec: results}
Here we present the results from our experiments on 
[REDACTED]-internal datasets. In Appendix A, we also provide experimental results for an open source  dataset, USS \citep{Sun:2021:SUS}, which  includes SGD, MultiWOZ, ReDial, and CCPE subsets.

\noindent \textbf{Larger model helps zero-shot dialogue evaluation.} 
In exploring the link between model size and zero-shot ability in dialogue quality evaluation, Table \ref{tab:model_size} presents Spearman and Pearson correlation values with human annotation across Alpaca, Llama, and Falcon series configurations.

Table ~\ref{tab:model_size} suggests a positive correlation between model size and zero-shot ability in dialogue quality evaluation. Notably, Falcon-40b shows a significant improvement (Spearman: -0.02 to 0.41), while the Llama series exhibits no significant improvement, possibly due to the original Llama's poor instruction understanding.

This conclusion underscores the potential benefits of employing larger models in dialogue systems, particularly for applications that require zero-shot flexibility. 
\begin{table}[t]
    \centering
    \large
    \caption{Performance comparison across model with different sizes on [REDACTED]-internal datasets. Spearman and Pearson correlation values presented, with the best results highlighted in bold.}
    \resizebox{0.49\textwidth}{!}{\begin{tabular}{l|cc|ccc|cc}
    \toprule
    Models                & Alpaca-7b & Alpaca-13b & Llama-7b & Llama-13b & Llama-30b & Falcon-7b-instruct & Falcon-40b-instruct \\
    \midrule
    Spearman correlation   & 0.47      & \textbf{0.48}       & 0.00     & 0.01     & \textbf{0.01}     & -0.02     & \textbf{0.41}       \\
    Pearson correlation    & 0.47      & \textbf{0.48}       & 0.03     & 0.02    & \textbf{0.03}     & -0.02     & \textbf{0.35}       \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:model_size}
    \vspace*{-3mm}
\end{table}

\noindent \textbf{Instruction-tuning helps zero-shot dialogue evaluation.}
Table~\ref{tab:model_size} also highlights our analysis of instruction fine-tuning's impact on zero-shot dialogue quality evaluation, focusing on the Alpaca and Llama model families. The Alpaca series, benefiting from instruction fine-tuning based on foundational Llama models, demonstrates superior performance, consistently showing higher Spearman and Pearson correlation coefficients. This emphasizes the crucial role of instruction tuning in enhancing dialogue evaluation. For instance, Alpaca-13b outperforms Llama-13b by 0.47 in Spearman correlation (Table~\ref{tab:model_size}). We hypothesize that instruction tuning refines LLMs' comprehension of instructions, optimizing task execution accuracy and efficiency. These results suggest the potential of tuning for nuanced dialogue understanding, paving the way for further research and development in this domain.

\noindent \textbf{In-context examples enhance the performance of dialogue evaluation.} In some of our early experiments with open-source datasets, we found that providing just 4 in-context examples can lead to a 30\% improvement on F1-score compared to zero-shot settings on 2 of 4 open-source datasets. In addition, algorithm-based selection methods result in notable performance improvements over random selection for in-context examples. We provide a more detailed summary of these experiments in the Appendix.

% %%% MOVE TO APPENDIX
% \begin{table*}[t]
% \centering
% \caption{Comparison of different in-context example selection methods and zero-shot ability for dialogue quality evaluation across different datasets using Falcon-7b-instruct Model on open-source dataset.}
% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{lcccccccccccccccc}
% \toprule
% Dataset & Model & Defect Rate & \multicolumn{3}{c}{Defect Class} & \multicolumn{3}{c}{Non-Defect Class} & \multicolumn{3}{c}{Weighted Average} & \multicolumn{3}{c}{Macro Average} & {Spearman} & Pearson \\
%         &       &             & Precision & Recall & F1-Score & Precision & Recall & F1-score & Precision & Recall & F1-score & Precision & Recall & F1-score\\
% \midrule
% \multirow{7}{*}{CCPE} & Zero-shot & 62\% & 0.71 & 0.39 & 0.5 & 0.42 & 0.74 & 0.54 & 0.6 & 0.52 & 0.51 & 0.57 & 0.56 & 0.52 & 0.21 & 0.27 \\
% &Random-1 & 62\% & 0.75 & 0.19 & 0.31 & 0.4 & \textbf{0.89} & 0.56 & 0.62 & 0.46 & 0.4 & 0.58 & 0.54 & 0.43 & \textbf{0.44} & 0.25 \\
% &BM25-1 & 62\% & \textbf{0.79} & 0.35 & 0.49 & 0.44 & 0.84 & \textbf{0.58} & 0.66 & 0.54 & 0.52 & 0.62 & 0.6 & 0.54 & 0.4 & \textbf{0.31} \\
% &Bert-1 & 62\% & 0.73 & 0.26 & 0.38 & 0.41 & 0.84 & 0.55 & 0.61 & 0.48 & 0.45 & 0.57 & 0.55 & 0.47 & 0.18 & 0.19 \\
% &Random-4 & 62\% & 0.71 & 0.55 & 0.62 & 0.46 & 0.63 & 0.53 & 0.61 & 0.58 & 0.59 & 0.58 & 0.59 & 0.58 & 0.16 & 0.17 \\
% &BM25-4 & 62\% & 0.73 & \textbf{0.77} & \textbf{0.75} & \textbf{0.59} & 0.53 & 0.56 & \textbf{0.67} & \textbf{0.68} & \textbf{0.68} & \textbf{0.66} & \textbf{0.65} & \textbf{0.65} & 0.23 & 0.2 \\
% &Bert-4 & 62\% & 0.68 & 0.68 & 0.68 & 0.47 & 0.47 & 0.47 & 0.6 & 0.6 & 0.6 & 0.58 & 0.58 & 0.58 & -0.07 & -0.13 \\
% \midrule
% \multirow{7}{*}{MWOZ} &Zero-shot & 55\% & 0.5 & 0.29 & 0.37 & 0.43 & 0.64 & 0.51 & 0.47 & 0.45 & 0.43 & 0.46 & 0.47 & 0.44 & -0.05 & 0.0 \\
% &Random-1 & 55\% & 0.55 & 0.11 & 0.18 & 0.45 & \textbf{0.89} & \textbf{0.6} & 0.5 & 0.46 & 0.37 & 0.5 & 0.5 & 0.39 & 0.09 & \textbf{0.1} \\
% &BM25-1 & 55\% & 0.53 & 0.15 & 0.23 & 0.45 & 0.84 & 0.58 & 0.49 & 0.46 & 0.39 & 0.49 & 0.49 & 0.41 & \textbf{0.18} & 0.06 \\
% &Bert-1 & 55\% & \textbf{0.63} & 0.18 & 0.28 & 0.46 & 0.87 & \textbf{0.6} & 0.55 & 0.49 & 0.43 & 0.54 & 0.52 & 0.44 & 0.13 & 0.0 \\
% &Random-4 & 55\% & 0.53 & 0.35 & 0.42 & 0.44 & 0.62 & 0.51 & 0.49 & 0.47 & 0.46 & 0.48 & 0.48 & 0.47 & 0.09 & 0.08 \\
% &BM25-4 & 55\% & 0.61 & \textbf{0.6} & \textbf{0.61} & \textbf{0.52} & 0.53 & 0.53 & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & 0.08 & 0.04 \\
% &Bert-4 & 55\% & 0.56 & 0.58 & 0.57 & 0.47 & 0.44 & 0.45 & 0.52 & 0.52 & 0.52 & 0.51 & 0.51 & 0.51 & 0.06 & 0.05 \\
% \midrule
% \multirow{7}{*}{Redial} & Zero-shot & 44\% & 0.49 & \textbf{0.55} & \textbf{0.52} & \textbf{0.61} & 0.55 & 0.58 & 0.56 & 0.55 & 0.55 & 0.55 & 0.55 & \textbf{0.55} & 0.09 & 0.11 \\
% &Random-1 & 44\% & 0.5 & 0.2 & 0.29 & 0.57 & \textbf{0.84} & 0.68 & 0.54 & 0.56 & 0.51 & 0.54 & 0.52 & 0.49 & 0.18 & 0.24 \\
% &BM25-1 & 44\% & 0.48 & 0.27 & 0.35 & 0.57 & 0.77 & 0.66 & 0.53 & 0.55 & 0.52 & 0.53 & 0.52 & 0.5 & 0.2 & 0.17 \\
% &Bert-1 & 44\% & \textbf{0.58} & 0.32 & 0.41 & \textbf{0.61} & 0.82 & \textbf{0.7} & \textbf{0.6} & \textbf{0.6} & \textbf{0.57} & \textbf{0.59} & \textbf{0.57} & \textbf{0.55} & \textbf{0.24} & \textbf{0.29} \\
% &Random-4 & 44\% & 0.5 & 0.41 & 0.45 & 0.59 & 0.68 & 0.63 & 0.55 & 0.56 & 0.55 & 0.55 & 0.54 & 0.54 & 0.12 & 0.11 \\
% &BM25-4 & 44\% & 0.4 & 0.45 & 0.43 & 0.52 & 0.46 & 0.49 & 0.47 & 0.46 & 0.46 & 0.46 & 0.46 & 0.46 & 0.1 & 0.15 \\
% &Bert-4 & 44\% & 0.44 & \textbf{0.55} & 0.49 & 0.57 & 0.46 & 0.51 & 0.51 & 0.5 & 0.5 & 0.5 & 0.5 & 0.5 & 0.05 & 0.05 \\
%                        \midrule
% \multirow{7}{*}{SGD} & Zero-shot & {48\%} & \textbf{0.64} & \textbf{0.63} & \textbf{0.63} & \textbf{0.66} & {0.67} & \textbf{0.67} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.34} & \textbf{0.32} \\
%                       & Random-1  & 48\% & 0.40 & 0.08 & 0.14 & 0.51 & \textbf{0.88} & 0.65 & 0.46 & 0.50 & 0.40 & 0.46 & 0.48 & 0.39 & 0.20 & 0.09 \\
%                       & BM25-1    & 48\% & 0.39 & 0.15 & 0.21 & 0.50 & 0.79 & 0.61 & 0.45 & 0.48 & 0.42 & 0.44 & 0.47 & 0.41 & 0.29 & 0.15 \\
%                       & Bert-1    & 48\% & 0.50 & 0.15 & 0.23 & 0.52 & 0.87 & 0.65 & 0.51 & 0.52 & 0.45 & 0.51 & 0.51 & 0.44 & 0.33 & 0.26 \\
%                       & Random-4  & 48\% & 0.44 & 0.33 & 0.38 & 0.50 & 0.62 & 0.55 & 0.47 & 0.48 & 0.47 & 0.47 & 0.47 & 0.47 & -0.01 & -0.02 \\
%                       & BM25-4    & 48\% & 0.52 & 0.58 & 0.55 & 0.57 & 0.50 & 0.53 & 0.54 & 0.54 & 0.54 & 0.54 & 0.54 & 0.54 & 0.06 & 0.08 \\
%                       & Bert-4    & 48\% & 0.37 & 0.40 & 0.38 & 0.41 & 0.38 & 0.40 & 0.39 & 0.39 & 0.39 & 0.39 & 0.39 & 0.39 & -0.12 & -0.12 \\


% \bottomrule
% \end{tabular}
% }
% \vspace*{-3mm}
% \label{tab:in-context-examples}
% \end{table*}

% \noindent \textbf{In-context examples enhance the performance of dialogue evaluation.}
% In this section, we evaluate the influence of in-context examples on the chosen base model, Falcon-7b-instruct, utilizing three distinct in-context example selection methods: Random, BM25, and Bert. These experiments are conducted on the open-sourced dataset USS shown in Table\,\ref{tab:in-context-examples}.

% First, it is evident that, in general, the few-shot performance demonstrates superiority over the zero-shot performance. A closer examination reveals that the best performance across various evaluation metrics is primarily concentrated within the few-shot settings in the first three datasets. If we take a closer look at the MWOZ dataset, all highlighted numbers are in the few-shots settings.    This observation substantiates the notion that providing in-context examples can indeed enhance the performance in dialogue evaluation. However, it is worth noting that an excessive provision of examples does not necessarily lead to further improvement. We hypothesize that this limitation may stem from the capacity constraints of LLMs, which can struggle to process overly lengthy inputs, occasionally resulting in performance degradation. This pattern is particularly evident in the Redial dataset, where the performance of the 4-shot approach does not surpass the results obtained from the 1-shot experiment. In addition to the findings presented, Table~\ref{tab:in-context-examples} reveals that the zero-shot performance outperforms the few-shot settings in the SGD dataset. This is likely attributable to the capacity constraints of LLMs; the dialogue lengths should not be excessively long. Notably, the dialogues in the SGD dataset have more turns ($26.7$ turns per dialogue) compared to the other three datasets from \citet{Sun:2021:SUS}. Such findings further emphasize the nuanced relationship between the number of in-context examples and the resultant performance, highlighting the importance of careful selection and optimization in applying few-shot learning techniques.

% Second, when comparing the performance across different in-context selection methods, we find that algorithm-based selection methods result in notable performance improvements over random selection for in-context examples. For instance, the BM25 and Bert methods consistently perform best across all datasets. Upon closer examination of the CCPE dataset in Table~\ref{tab:in-context-examples}, we observe that $85\%$ of the highest values across all metrics are derived from the algorithm's selected method. What is more, the optimal choice for selecting different in-context example methods varies based on the dataset. In the first two datasets, the BM25 method excels, while in the third, the Bert method stands out.

% In conclusion, our results suggest that in-context examples can significantly enhance the quality of dialogue evaluation. Our findings also underscore the importance of employing algorithmic methods for selecting these examples, as the right selection strategy can lead to meaningful performance gains. By revealing these patterns, our study contributes to a deeper understanding of how few-shot learning can be best utilized in dialogue systems.


\begin{table}[hbt!]
\centering
\caption{Summary of performance metrics for supervised finetuning models on [REDACTED]-internal datasets across different training datasets and various model architectures.}
\vspace*{-3mm}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline

Models           & Spearman & Pearson & Precision& Recall & F1\ & F1-micro \\
\hline
Alpaca-7b          & 0.47     & 0.47    & 0.52             & \textbf{0.72}          & 0.60      & \textbf{0.69} \\
Alpaca-7b-sft-small & 0.61     & 0.61    & \textbf{0.96}             & 0.59          & \textbf{0.73}      & {0.65} \\
Alpaca-7b-sft-large & \textbf{0.64}     & \textbf{0.66}    & 0.93             & 0.58          & 0.72      & 0.33 \\
\midrule
Llama-7b           & 0.00     & 0.03    & 0.67             & \textbf{1.00}          & \textbf{0.80}      & 0.33 \\
Llama-7b-sft-small & 0.58     & 0.60    & 0.92             & 0.62          & 0.74      & \textbf{0.58} \\
Llama-7b-sft-large & \textbf{0.64}     & \textbf{0.66}    & 0.93             & 0.58          & 0.72      & 0.33 \\
\midrule
Llama-13b          & 0.01    & 0.02   & 0.67             & \textbf{1.00}          & \textbf{0.80}      & 0.36 \\
Llama-13b-sft-small & 0.64     & 0.65    & 0.94             & 0.61          & 0.74      & \textbf{0.46} \\
Llama-13b-sft-large & \textbf{0.64}     & \textbf{0.65}    & 0.97             & 0.54          & 0.69      & 0.40 \\
\midrule
Falcon-40b-instruct         & 0.41     & 0.36    & \textbf{1.00}             & 0.01          & 0.02      & 0.67 \\
Falcon-40b-instruct-sft-small   & 0.60     & 0.61    & 0.96             & 0.52          & 0.67      & 0.65 \\
Falcon-40b-instruct-sft-large   & \textbf{0.61}     & \textbf{0.63}    & 0.93             & \textbf{0.53}          & \textbf{0.68}      & \textbf{0.69} \\
\midrule
\hline
\end{tabular}}

\label{tab:sft_results}
\end{table}

\begin{table*}[bt]
\centering
\small
\caption{\footnotesize{Comparison of two Chain-of-Thought Methods on the internal dataset over Falcon-7b-instruct model. The 'Rating-first' method refers to generating the score first, followed by the reasons, while the 'Analysis-first' method involves generating an analysis first, then determining the scores. The Defect Class category means computation of corresponding metrics specifically for the defect class. Experiments are conducted on the [REDACTED]-internal datasets.}}
\vspace*{-3mm}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{lccccccccccccccc}
\toprule
Model & Defect Rate & \multicolumn{3}{c}{Defect Class} & \multicolumn{3}{c}{Non-Defect Class} & \multicolumn{3}{c}{Weighted Average} & \multicolumn{3}{c}{Macro Average} & Spearman & Pearson \\
 & & Precision & Recall & F1-Score & Precision & Recall & F1-score & Precision & Recall & F1-score & Precision & Recall & F1-score & & \\
\midrule
Rating-first & 59\% & 0.59 & \textbf{1.00} & 0.74 & \textbf{0.67} & 0.01 & 0.02 & 0.62 & 0.59 & 0.45 & 0.63 & 0.50 & 0.38 & 0.10 & 0.07 \\
Analysis-first & 59\% & \textbf{0.67} & {0.86} & \textbf{0.75} & 0.66 & \textbf{0.39} & \textbf{0.49} & \textbf{0.67} & \textbf{0.67} & \textbf{0.65} & \textbf{0.67} & \textbf{0.63} & \textbf{0.62} & \textbf{0.23} & \textbf{0.28} \\
\bottomrule
\end{tabular}}
\vspace*{-3mm}
\label{tab:resaons_ratings}
\end{table*}

\noindent \textbf{How supervised fine-tuning influence the prediction results.}
In this section, we examine the influence of supervised fine-tuning on the performance of LLMs for the dialogue evaluation task. Our analysis involves leveraging two internal datasets used for training dialog quality estimation models. The first is a small version of the dataset, resulting in models denoted as "xxx-small," while the second is a larger version, leading to models labeled as "xxx-large."

We report on several performance metrics, including precision, recall, F1-score, and F1-micro, in accordance with the settings delineated in \citet{komma2023toward}. Our findings from Table\,\ref{tab:sft_results} reveal a consistent improvement in the original model's performance after supervised fine-tuning, especially in the Spearman and Pearson correlations with human annotation. For instance, the model "Falcon-40b-instruct-sft-large" exhibits a $48\%$ relative improvement compared to the original "Falcon-40b-instruct." This indicates that supervised fine-tuning enhances the alignment of the model's scoring with human evaluation. 

Furthermore, an analysis of F1-micro reveals that supervised fine-tuning generally augments performance in comparison to the original model. For instance, when comparing the Llama-7b-sft-small to the original Llama-7b, there is a $75\%$ relative improvement. A closer examination of the data also suggests that utilizing a larger dataset can boost overall performance. For example, the highest correlations in the first two columns are consistently associated with models trained on the larger dataset. Interestingly, models trained on smaller datasets occasionally exhibit superior F1-micro scores, as observed in the "Llama" series. For example, when comparing the Llama-13b-sft-small to the original Llama-13b-sft-large, there is a $15\%$ relative improvement. We hypothesize that this may occur when the score distribution between the small dataset and the test dataset aligns more closely shown in Figure~\ref{fig: score_distribution}.

In conclusion, our findings affirm that supervised fine-tuning can substantially enhance the performance of large language models compared to their original configurations. This study underscores the value of fine-tuning and dataset selection in achieving more accurate and human-aligned evaluations in the context of dialogue systems.


\noindent \textbf{Chain-of-thought for generation score and reasons.} In this section, we shift our focus to the utilization of the "generation and chain-of-thought" approach, which not only generates scores but also provides reasons for selecting those scores. We explore two distinct paradigms to accomplish this task. The first paradigm involves prompting the LLMs to generate an analysis first and then derive ratings based on that analysis, named \textbf{Analysis-first}. The second paradigm, conversely, prompts the LLMs to generate a rating first and then elucidate the reasons for choosing that particular score, named \textbf{Rating-first}.

Interestingly, our findings suggest that the first paradigm—analysis, then rating (Analysis-first), provides more aligned scores and reasons, as demonstrated in Table \ref{tab:resaons_ratings}. We observe a consistent improvement compared to the approach of generating a rating first and then providing reasons (Rating-first). For example, Analysis-first methods outperform Rating-first in $85\%$ of all evaluation metrics. Upon conducting a failure analysis, we discovered that in the cases where a rating is generated first, the scores do not always align with the subsequent reasons. However, in the paradigm where the analysis is generated first, followed by the rating, there is a consistent alignment between ratings and scores. We attribute the observed improvement to this consistency.

The implications of these findings may extend to various applications where the alignment between scores and reasoning is essential. Further exploration of these paradigms and their potential advantages and limitations may provide valuable insights into the optimal utilization of LLMs for complex tasks such as rating and explanation generation. %The details of prompts we used are listed in the Sec\,\ref{sec: prompts}.


==> tex/_clutter/Experiment_results_old.tex <==
\section{Results}
\label{sec: results}
\noindent \textbf{Larger model helps zero-shot dialogue evaluation.} 
When examining the relationship between model size and zero-shot ability in dialogue quality evaluation, Table\,\ref{tab:model_size} displays Spearman and Pearson correlation values with human annotation for different model configurations across the Alpaca, Llama, and Falcon series.

The empirical evidence provided by the Table\,\ref{tab:model_size}  suggests a positive relationship between model size and zero-shot ability in dialogue quality evaluation. For example, there is a significant improvement  observed in the Falcon series, where the Spearman correlation shifts from -0.02 for Falcon-7b to 0.41 for Falcon-40b. While the effect's magnitude may vary, the trend is evident across different series. For example, there is no significant improvement in the Llama series, same pearson correlation on the Llama-7 and Llama-30b), but they all performs bad on this task. The reason might be the poor ability of original Llama to understand instruction.

This conclusion underscores the potential benefits of employing larger models in dialogue systems, particularly for applications that require zero-shot flexibility. 
\begin{table}[t]
    \centering
    \large
    \caption{Performance comparison across model with different sizes on Amazon-internal datasets. Spearman and Pearson correlation values presented, with the best results highlighted in bold.}
    \resizebox{0.49\textwidth}{!}{\begin{tabular}{l|cc|ccc|cc}
    \toprule
    Models                & Alpaca-7b & Alpaca-13b & Llama-7b & Llama-13b & Llama-30b & Falcon-7b-instruct & Falcon-40b-instruct \\
    \midrule
    Spearman correlation   & 0.47      & \textbf{0.48}       & 0.00     & 0.01     & \textbf{0.01}     & -0.02     & \textbf{0.41}       \\
    Pearson correlation    & 0.47      & \textbf{0.48}       & 0.03     & 0.02    & \textbf{0.03}     & -0.02     & \textbf{0.35}       \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:model_size}
    \vspace*{-3mm}
\end{table}

\noindent \textbf{Instruction-tuning helps zero-shot dialogue evaluation.}
Table~\ref{tab:model_size}  also presents our results on analyzing the impact of instruction fine-tuning on models' ability to do zero-shot dialogue quality evaluation. For this study, we  primarily focus on two model families, Alpaca and Llama. It is noteworthy that the Alpaca series underwent instruction fine-tuning based on the foundational Llama models, an important modification to enhance performance. Our empirical findings illuminate the comparative superiority of the Alpaca models in the realm of zero-shot dialogue quality evaluation, as evidenced by consistently elevated Spearman and Pearson correlation coefficients. This observation underscores the significance of instruction tuning as a critical technological approach for augmenting dialogue evaluation performance. For example, the improvement from Alpaca-13b compared to the Llama-13b models is 0.47 on the Spearman correlation shown in Table~\ref{tab:model_size}. We hypothesize that instruction tuning may serve to refine LLMs comprehension of instructions or prompts, thereby optimizing their ability to execute the specified tasks with greater accuracy and efficiency. The results suggest that such tuning may be instrumental in facilitating a more nuanced understanding of dialogues, opening promising avenues for further research and development in this domain.
\begin{table*}[t]
\centering
\caption{Comparison of different in-context example selection methods and zero-shot ability for dialogue quality evaluation across different datasets using Falcon-7b-instruct Model on open-source dataset.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccccccccccccc}
\toprule
Dataset & Model & Defect Rate & \multicolumn{3}{c}{Defect Class} & \multicolumn{3}{c}{Non-Defect Class} & \multicolumn{3}{c}{Weighted Average} & \multicolumn{3}{c}{Macro Average} & {Spearman} & Pearson \\
        &       &             & Precision & Recall & F1-Score & Precision & Recall & F1-score & Precision & Recall & F1-score & Precision & Recall & F1-score\\
\midrule
\multirow{7}{*}{CCPE} & Zero-shot & 62\% & 0.71 & 0.39 & 0.5 & 0.42 & 0.74 & 0.54 & 0.6 & 0.52 & 0.51 & 0.57 & 0.56 & 0.52 & 0.21 & 0.27 \\
&Random-1 & 62\% & 0.75 & 0.19 & 0.31 & 0.4 & \textbf{0.89} & 0.56 & 0.62 & 0.46 & 0.4 & 0.58 & 0.54 & 0.43 & \textbf{0.44} & 0.25 \\
&BM25-1 & 62\% & \textbf{0.79} & 0.35 & 0.49 & 0.44 & 0.84 & \textbf{0.58} & 0.66 & 0.54 & 0.52 & 0.62 & 0.6 & 0.54 & 0.4 & \textbf{0.31} \\
&BERT-1 & 62\% & 0.73 & 0.26 & 0.38 & 0.41 & 0.84 & 0.55 & 0.61 & 0.48 & 0.45 & 0.57 & 0.55 & 0.47 & 0.18 & 0.19 \\
&Random-4 & 62\% & 0.71 & 0.55 & 0.62 & 0.46 & 0.63 & 0.53 & 0.61 & 0.58 & 0.59 & 0.58 & 0.59 & 0.58 & 0.16 & 0.17 \\
&BM25-4 & 62\% & 0.73 & \textbf{0.77} & \textbf{0.75} & \textbf{0.59} & 0.53 & 0.56 & \textbf{0.67} & \textbf{0.68} & \textbf{0.68} & \textbf{0.66} & \textbf{0.65} & \textbf{0.65} & 0.23 & 0.2 \\
&BERT-4 & 62\% & 0.68 & 0.68 & 0.68 & 0.47 & 0.47 & 0.47 & 0.6 & 0.6 & 0.6 & 0.58 & 0.58 & 0.58 & -0.07 & -0.13 \\
\midrule
\multirow{7}{*}{MWOZ} &Zero-shot & 55\% & 0.5 & 0.29 & 0.37 & 0.43 & 0.64 & 0.51 & 0.47 & 0.45 & 0.43 & 0.46 & 0.47 & 0.44 & -0.05 & 0.0 \\
&Random-1 & 55\% & 0.55 & 0.11 & 0.18 & 0.45 & \textbf{0.89} & \textbf{0.6} & 0.5 & 0.46 & 0.37 & 0.5 & 0.5 & 0.39 & 0.09 & \textbf{0.1} \\
&BM25-1 & 55\% & 0.53 & 0.15 & 0.23 & 0.45 & 0.84 & 0.58 & 0.49 & 0.46 & 0.39 & 0.49 & 0.49 & 0.41 & \textbf{0.18} & 0.06 \\
&BERT-1 & 55\% & \textbf{0.63} & 0.18 & 0.28 & 0.46 & 0.87 & \textbf{0.6} & 0.55 & 0.49 & 0.43 & 0.54 & 0.52 & 0.44 & 0.13 & 0.0 \\
&Random-4 & 55\% & 0.53 & 0.35 & 0.42 & 0.44 & 0.62 & 0.51 & 0.49 & 0.47 & 0.46 & 0.48 & 0.48 & 0.47 & 0.09 & 0.08 \\
&BM25-4 & 55\% & 0.61 & \textbf{0.6} & \textbf{0.61} & \textbf{0.52} & 0.53 & 0.53 & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & \textbf{0.57} & 0.08 & 0.04 \\
&BERT-4 & 55\% & 0.56 & 0.58 & 0.57 & 0.47 & 0.44 & 0.45 & 0.52 & 0.52 & 0.52 & 0.51 & 0.51 & 0.51 & 0.06 & 0.05 \\
\midrule
\multirow{7}{*}{Redial} & Zero-shot & 44\% & 0.49 & \textbf{0.55} & \textbf{0.52} & \textbf{0.61} & 0.55 & 0.58 & 0.56 & 0.55 & 0.55 & 0.55 & 0.55 & \textbf{0.55} & 0.09 & 0.11 \\
&Random-1 & 44\% & 0.5 & 0.2 & 0.29 & 0.57 & \textbf{0.84} & 0.68 & 0.54 & 0.56 & 0.51 & 0.54 & 0.52 & 0.49 & 0.18 & 0.24 \\
&BM25-1 & 44\% & 0.48 & 0.27 & 0.35 & 0.57 & 0.77 & 0.66 & 0.53 & 0.55 & 0.52 & 0.53 & 0.52 & 0.5 & 0.2 & 0.17 \\
&BERT-1 & 44\% & \textbf{0.58} & 0.32 & 0.41 & \textbf{0.61} & 0.82 & \textbf{0.7} & \textbf{0.6} & \textbf{0.6} & \textbf{0.57} & \textbf{0.59} & \textbf{0.57} & \textbf{0.55} & \textbf{0.24} & \textbf{0.29} \\
&Random-4 & 44\% & 0.5 & 0.41 & 0.45 & 0.59 & 0.68 & 0.63 & 0.55 & 0.56 & 0.55 & 0.55 & 0.54 & 0.54 & 0.12 & 0.11 \\
&BM25-4 & 44\% & 0.4 & 0.45 & 0.43 & 0.52 & 0.46 & 0.49 & 0.47 & 0.46 & 0.46 & 0.46 & 0.46 & 0.46 & 0.1 & 0.15 \\
&BERT-4 & 44\% & 0.44 & \textbf{0.55} & 0.49 & 0.57 & 0.46 & 0.51 & 0.51 & 0.5 & 0.5 & 0.5 & 0.5 & 0.5 & 0.05 & 0.05 \\
                       \midrule
\multirow{7}{*}{SGD} & Zero-shot & {48\%} & \textbf{0.64} & \textbf{0.63} & \textbf{0.63} & \textbf{0.66} & {0.67} & \textbf{0.67} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.65} & \textbf{0.34} & \textbf{0.32} \\
                      & Random-1  & 48\% & 0.40 & 0.08 & 0.14 & 0.51 & \textbf{0.88} & 0.65 & 0.46 & 0.50 & 0.40 & 0.46 & 0.48 & 0.39 & 0.20 & 0.09 \\
                      & BM25-1    & 48\% & 0.39 & 0.15 & 0.21 & 0.50 & 0.79 & 0.61 & 0.45 & 0.48 & 0.42 & 0.44 & 0.47 & 0.41 & 0.29 & 0.15 \\
                      & BERT-1    & 48\% & 0.50 & 0.15 & 0.23 & 0.52 & 0.87 & 0.65 & 0.51 & 0.52 & 0.45 & 0.51 & 0.51 & 0.44 & 0.33 & 0.26 \\
                      & Random-4  & 48\% & 0.44 & 0.33 & 0.38 & 0.50 & 0.62 & 0.55 & 0.47 & 0.48 & 0.47 & 0.47 & 0.47 & 0.47 & -0.01 & -0.02 \\
                      & BM25-4    & 48\% & 0.52 & 0.58 & 0.55 & 0.57 & 0.50 & 0.53 & 0.54 & 0.54 & 0.54 & 0.54 & 0.54 & 0.54 & 0.06 & 0.08 \\
                      & BERT-4    & 48\% & 0.37 & 0.40 & 0.38 & 0.41 & 0.38 & 0.40 & 0.39 & 0.39 & 0.39 & 0.39 & 0.39 & 0.39 & -0.12 & -0.12 \\


\bottomrule
\end{tabular}
}
\vspace*{-3mm}
\label{tab:in-context-examples}
\end{table*}

\noindent \textbf{In-context examples enhance the performance of dialogue evaluation.}
In this section, we evaluate the influence of in-context examples on the chosen base model, Falcon-7b-instruct, utilizing three distinct in-context example selection methods: Random, BM25, and BERT. For the BM25 and BERT-based ICL approaches, we selected either 1 or 4 of the most semantically similar examples from the training set. The selection was based on the semantic similarity between the examples, as determined by the BM25 and BERT models. In contrast, for the Random-based ICL approach, we randomly picked either 1 or 4 examples from the training set to use as the in-context examples. These experiments are conducted on the open-sourced dataset USS shown in Table\,\ref{tab:in-context-examples}.

First, it is evident that, in general, the few-shot performance demonstrates superiority over the zero-shot performance. A closer examination reveals that the best performance across various evaluation metrics is primarily concentrated within the few-shot settings in the first three datasets. If we take a closer look at the MWOZ dataset, all highlighted numbers are in the few-shots settings.    This observation substantiates the notion that providing in-context examples can indeed enhance the performance in dialogue evaluation. However, it is worth noting that an excessive provision of examples does not necessarily lead to further improvement. We hypothesize that this limitation may stem from the capacity constraints of LLMs, which can struggle to process overly lengthy inputs, occasionally resulting in performance degradation. This pattern is particularly evident in the Redial dataset, where the performance of the 4-shot approach does not surpass the results obtained from the 1-shot experiment. In addition to the findings presented, Table~\ref{tab:in-context-examples} reveals that the zero-shot performance outperforms the few-shot settings in the SGD dataset. This is likely attributable to the capacity constraints of LLMs; the dialogue lengths should not be excessively long. Notably, the dialogues in the SGD dataset have more turns ($26.7$ turns per dialogue) compared to the other three datasets from \citet{Sun:2021:SUS}. Such findings further emphasize the nuanced relationship between the number of in-context examples and the resultant performance, highlighting the importance of careful selection  in  few-shot learning.

Second, when comparing the performance across different in-context selection methods, we find that algorithm-based selection methods result in notable performance improvements over random selection for in-context examples. For instance, the BM25 and BERT methods consistently perform best across all datasets. Upon closer examination of the CCPE dataset in Table~\ref{tab:in-context-examples}, we observe that $85\%$ of the highest values across all metrics are derived from the algorithm's selected method. What is more, the optimal choice for selecting different in-context example methods varies based on the dataset. In the first two datasets, the BM25 method excels, while in the third, the BERT method stands out.

In conclusion, our results suggest that in-context examples can significantly enhance the quality of dialogue evaluation. Our findings also underscore the importance of employing algorithmic methods for selecting these examples, as the right selection strategy can lead to meaningful performance gains. By revealing these patterns, our study contributes to a deeper understanding of how few-shot learning can be best utilized in dialogue systems.
\begin{table}[hbt!]
\centering
\caption{Summary of performance metrics for supervised finetuning models on Amazon-internal datasets across different training datasets and various model architectures.}
\vspace*{-3mm}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline

Models           & Spearman & Pearson & Precision& Recall & F1\ & F1-micro \\
\hline
Alpaca-7b          & 0.47     & 0.47    & 0.52             & \textbf{0.72}          & 0.60      & \textbf{0.69} \\
Alpaca-7b-sft-small & 0.61     & 0.61    & \textbf{0.96}             & 0.59          & \textbf{0.73}      & {0.65} \\
Alpaca-7b-sft-large & \textbf{0.64}     & \textbf{0.66}    & 0.93             & 0.58          & 0.72      & 0.33 \\
\midrule
Llama-7b           & 0.00     & 0.03    & 0.67             & \textbf{1.00}          & \textbf{0.80}      & 0.33 \\
Llama-7b-sft-small & 0.58     & 0.60    & 0.92             & 0.62          & 0.74      & \textbf{0.58} \\
Llama-7b-sft-large & \textbf{0.64}     & \textbf{0.66}    & 0.93             & 0.58          & 0.72      & 0.33 \\
\midrule
Llama-13b          & 0.01    & 0.02   & 0.67             & \textbf{1.00}          & \textbf{0.80}      & 0.36 \\
Llama-13b-sft-small & 0.64     & 0.65    & 0.94             & 0.61          & 0.74      & \textbf{0.46} \\
Llama-13b-sft-large & \textbf{0.64}     & \textbf{0.65}    & 0.97             & 0.54          & 0.69      & 0.40 \\
\midrule
Falcon-40b-instruct         & 0.41     & 0.36    & \textbf{1.00}             & 0.01          & 0.02      & 0.67 \\
Falcon-40b-instruct-sft-small   & 0.60     & 0.61    & 0.96             & 0.52          & 0.67      & 0.65 \\
Falcon-40b-instruct-sft-large   & \textbf{0.61}     & \textbf{0.63}    & 0.93             & \textbf{0.53}          & \textbf{0.68}      & \textbf{0.69} \\
\midrule
\hline
\end{tabular}}

\label{tab:sft_results}
\end{table}



\noindent \textbf{How supervised fine-tuning influence the prediction results.}
Here we examine the influence of supervised fine-tuning on the performance of LLMs for the dialogue evaluation task. Specifically, we fine-tuned the models using both Likert-scale and binary label data. We leverage two internal datasets used for training dialog quality estimation models. The first is a small version of the dataset, resulting in models denoted as "xxx-small," while the second is a larger version, leading to models labeled as "xxx-large."

We report on several performance metrics, including precision, recall, F1-score, and F1-micro, in accordance with the settings delineated in \citet{komma2023toward}. Our findings from Table\,\ref{tab:sft_results} reveal a consistent improvement in the original model's performance after supervised fine-tuning, especially in the Spearman and Pearson correlations with human annotation. For instance, the model ``Falcon-40b-instruct-sft-large'' exhibits a $48\%$ relative improvement compared to the original ``Falcon-40b-instruct.'' This indicates that supervised fine-tuning enhances the alignment of the model's scoring with human evaluation. 

Furthermore, an analysis of F1-micro reveals that supervised fine-tuning generally augments performance in comparison to the original model. For instance, when comparing the Llama-7b-sft-small to the original Llama-7b, there is a $75\%$ relative improvement. A closer examination also suggests that utilizing a larger dataset can boost overall performance. For example, the highest correlations in the first two columns are consistently associated with models trained on the larger dataset. Interestingly, models trained on smaller datasets occasionally exhibit superior F1-micro scores, as for the "Llama" series. For example, when comparing the Llama-13b-sft-small to the original Llama-13b-sft-large, there is a $15\%$ relative improvement. We hypothesize that this may occur when the score distribution between the small dataset and the test dataset aligns more closely shown in Figure~\ref{fig: score_distribution}.
\begin{table*}[!h]
\centering
\small
\caption{\footnotesize{Comparison of Two Chain-of-Thoughts Methods on the internal dataset over Falcon-7b-instruct model. The 'Rating-first' method refers to generating the score first, followed by the reasons, while the 'Analysis-first' method involves generating an analysis first, then determining the scores. The Defect Class category means computation of corresponding metrics specifically for the defect class. Experiments are conducted on the Amazon-internal datasets.}}
\vspace*{-3mm}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{lccccccccccccccc}
\toprule
Model & Defect Rate & \multicolumn{3}{c}{Defect Class} & \multicolumn{3}{c}{Non-Defect Class} & \multicolumn{3}{c}{Weighted Average} & \multicolumn{3}{c}{Macro Average} & Spearman & Pearson \\
 & & Precision & Recall & F1-Score & Precision & Recall & F1-score & Precision & Recall & F1-score & Precision & Recall & F1-score & & \\
\midrule
Rating-first & 59\% & 0.59 & \textbf{1.00} & 0.74 & \textbf{0.67} & 0.01 & 0.02 & 0.62 & 0.59 & 0.45 & 0.63 & 0.50 & 0.38 & 0.10 & 0.07 \\
Analysis-first & 59\% & \textbf{0.67} & {0.86} & \textbf{0.75} & 0.66 & \textbf{0.39} & \textbf{0.49} & \textbf{0.67} & \textbf{0.67} & \textbf{0.65} & \textbf{0.67} & \textbf{0.63} & \textbf{0.62} & \textbf{0.23} & \textbf{0.28} \\
\bottomrule
\end{tabular}}
\vspace*{-3mm}
\label{tab:resaons_ratings}
\end{table*}
It's important to note that the Llama-7b and Llama-13b models predict defects for all test samples, which results in a recall of $1.0$ and a precision of $0.67$. However, this does not necessarily indicate optimal performance. To better understand the correlation between the model predictions and the ground truth, we should also consider the Spearman and Pearson correlations over likert scores, which provide more insight into the linear relationship between the predictions and the actual data.

In conclusion, our findings affirm that supervised fine-tuning can substantially enhance the performance of large language models compared to their original configurations. This study underscores the value of fine-tuning and dataset selection in achieving more accurate and human-aligned evaluations in the context of dialogue systems.


\noindent \textbf{Chain-of-thoughts for generation score and reasons.} In this section, we shift our focus to the utilization of the "generation and chain-of-thoughts" approach, which not only generates scores but also provides reasons for selecting those scores. We explore two distinct paradigms to accomplish this task. The first paradigm, \textbf{Analysis-first},  involves prompting the LLMs to generate an analysis first and then derive ratings based on that analysis. Conversely, the second paradigm, \textbf{Rating-first}, prompts the LLMs to generate a rating first and then elucidate the reasons for choosing that particular score; we refer the reader to Section~\ref{sec: prompts} for respective prompts. 

Interestingly, our findings suggest that the first paradigm—analysis, then rating (Analysis-first), provides more aligned scores and reasons, as demonstrated in Table \ref{tab:resaons_ratings}. We observe a consistent improvement compared to the approach of generating a rating first and then providing reasons (Rating-first). For example, Analysis-first methods outperform Rating-first in $85\%$ of all evaluation metrics. Upon conducting a failure analysis, we discovered that in the cases where a rating is generated first, the scores do not always align with the subsequent reasons. However, in the paradigm where the analysis is generated first, followed by the rating, there is a consistent alignment between ratings and scores. We attribute the observed improvement to this consistency.

The implications of these findings may extend to various applications where the alignment between scores and reasoning is essential. Further exploration of these paradigms and their potential advantages and limitations may provide valuable insights into the optimal utilization of LLMs for complex tasks such as rating and explanation generation. %The details of prompts we used are listed in the Sec\,\ref{sec: prompts}.


==> tex/_clutter/Experiment_setup-also-old.tex <==
\section{Experiment setup}

\noindent \textbf{Model.} 
In this study, we utilize models from the Llama family \citep{touvron2023llama} and the Falcon models series~\citep{falcon40b}. Additionally, we incorporate the instruction tuning variants of these models as proposed in the Alpaca study \cite{alpaca}. We set the temperature as $0.7$. \\
\noindent \textbf{Dataset.}

%%% <MOVE TO APPENDIX>
%We experiment on two datasets: USS \citep{Sun:2021:SUS} includes SGD, MultiWOZ, ReDial, and CCPE subsets, with a 1-5 score scale. We randomly allocate $10\%$ as test data, using the rest for training applicable to both supervised fine-tuning and in-context learning. Additionally, we evaluate our methods on internal datasets, using two versions of [REDACTED], with a similar 1-5 score scale \citep{komma2023toward}. The score distribution is shown in Figure \ref{fig: score_distribution}, with the smaller training set resembling the test set more closely than the larger one.
%%%

We experiment on two versions of an internal proprietary dataset of dialogs [REDACTED], which has a human annotated score on a scale of 1 to 5. The score distribution is shown in Figure \ref{fig: score_distribution}, with the smaller training set resembling the test set more closely than the larger one.

We binarize the datasets, considering scores below three as "defect" (unsatisfactory) and scores of three or above as "non-defect" (satisfactory). This binary classification scheme enables us to compute metrics for evaluating our approach and gaining insights into the effectiveness of our methods.
\begin{figure}[h]
\vspace*{-3mm}
\centerline{
\begin{tabular}{ccc}
    \hspace*{-2mm}  \includegraphics[width=25mm,height=!]{Figs/small_train.jpg} &
    \hspace*{-5mm} \includegraphics[width=25mm,height=!]{Figs/large_train.jpg} &
    \hspace*{-5mm} \includegraphics[width=25mm,height=!]{Figs/test.jpg} \\
    \hspace*{-2mm} (a) small train & \hspace*{-4mm}(b) large train & \hspace*{-5mm}(c) test
\end{tabular}
}
\vspace*{-2mm}
\caption{ Score distribution for the different train and test dataset over [REDACTED] internal dataset.
}
 \label{fig: score_distribution}
 \vspace*{-4mm}
\end{figure}
\\
\noindent \textbf{In-context example selection methods.}
In our paper, we use three methods to select in-context examples, enhancing model performance. The first is a random selection process from the training dataset. The second employs a probabilistic algorithm for information retrieval (IR) \citep{robertson2009probabilistic}, selecting similar examples based on a defined similarity metric. The third relies on BERT \citep{devlin2018bert}, extracting representations from the input dialogue and identifying similar examples using cosine similarity computations. These methods offer diverse strategies for in-context example selection, catering to various requirements and use cases. We conducted three runs for the random selection method and report the mean value. \\ 

\noindent \textbf{Supervised fine-tuning method.} In our study, we explore supervised fine-tuning on the training dataset for large language models. To manage computational costs, we adopt the Lora setting \citep{hu2021lora}, fine-tuning only a small number of parameters. This efficiently enhances the model's effectiveness while addressing computational challenges.

==> tex/_clutter/Experiment_setup_old.tex <==
\section{Experiment setup}

\noindent \textbf{Model.} 
In this study, we utilize models from the Llama family \citep{touvron2023llama} and the Falcon-40B models \citep{falcon40b}.\footnote{Most recent model at the time of the experiment.} Due to the sensitive nature of the internal dataset used in our experiments, we refrained from using closed-source LLMs such as ChatGPT. Additionally, we incorporate the instruction tuning variants of these models as proposed in the Alpaca study \cite{alpaca}. We set the temperature to $0.7$ during generation. \\
\noindent \textbf{Dataset.}
We focus on two distinct datasets in our experiments. The first one is the publicly available USS \citep{Sun:2021:SUS}, encompassing four English-based subsets: SGD, MultiWOZ, ReDial, and CCPE. This dataset employs a score scale ranging from 1 to 5. For our study, we randomly allocated 
$10\%$ of this dataset as test data, with the remainder serving as the training dataset. The training data is applicable for both supervised fine-tuning and in-context learning purposes.
In addition to the USS dataset, we evaluate the effectiveness of our methods on an Amazon-internal dataset, which also utilize a 1-5 score scale (similar in format to the data described in \citet{komma2023toward}). We incorporate two different versions of the Amazon-internal dataset for training in this research. The score distribution across these three internal datasets is illustrated in Figure \ref{fig: score_distribution}, where we can observe that the distribution of the smaller training set resembles the test set more closely than that of the larger training set.

We perform binarization on these two datasets, defining scores below three as ``defect'' (unsatisfactory) and scores of three or above as ``non-defect'' (satisfactory). This binary classification scheme allows us to compute relevant metrics to evaluate our approach, providing additional insights into the effectiveness of our methods.
\begin{figure}[h]
\vspace*{-3mm}
\centerline{
\begin{tabular}{ccc}
    \hspace*{-2mm}  \includegraphics[width=25mm,height=!]{Figs/small_train.jpg} &
    \hspace*{-5mm} \includegraphics[width=25mm,height=!]{Figs/large_train.jpg} &
    \hspace*{-5mm} \includegraphics[width=25mm,height=!]{Figs/test.jpg} \\
    \hspace*{-2mm} (a) small train & \hspace*{-4mm}(b) large train & \hspace*{-5mm}(c) test
\end{tabular}
}
\vspace*{-2mm}
\caption{ Score distribution for the different train and test splits over the Amazon-internal dataset.
}
 \label{fig: score_distribution}
 \vspace*{-4mm}
\end{figure}
\\
\noindent \textbf{In-context example selection methods.}
In our paper, we employ three distinct methods to select in-context examples, aiming to enhance model performance. The first method is a random selection process that chooses in-context examples arbitrarily from the training dataset. The second method leverages a probabilistic algorithm commonly used for information retrieval (IR) purposes called BM25 \citep{robertson2009probabilistic}. This approach selects the most similar examples as in-context ones based on a defined similarity metric. Finally, the third method relies on the BERT model \citep{devlin2018bert}. This approach extracts representations from the input dialogue and identifies the most similar examples within the training dataset based on cosine similarity computations. Together, these three methods offer diverse strategies for in-context example selection, catering to different requirements and use cases. We have ran for three times for the random selection methods, and report the mean value of it. \\ 
\noindent \textbf{Supervised fine-tuning method.} In our study, we also explore the use of supervised fine-tuning on the training dataset, investigating the effects and benefits of such methods with large language models. Recognizing the substantial computational cost associated with fully fine-tuning these models, we employ the Lora setting \citep{hu2021lora}. This approach allows us to achieve satisfactory performance by fine-tuning only a small number of parameters within the model. It serves as an efficient alternative that mitigates the computational challenges while still enhancing the model's effectiveness.

==> tex/outline.tex <==

\begin{center}
    \textbf{Outline of the paper}
\end{center}
\begin{enumerate}
    \item \textbf{Introduction.}  Considering to include the following paragraphs/topics
    \begin{enumerate}
        \item What is the dialog evaluation, and challenges for it?
        \item What is the LLMs recently and what the ability and strength for those LLMs. 
        \item Motivation for utilizing LLMs to do dialogue evaluation.
        \item Briefly review the most relevant works if any and state our \textbf{contributions}.
        \textbf{Remark:} We need a 
        \textbf{Figure} in Introduction to highlight how to utilize LLMs to fulfill dialog evaluation. 
    \end{enumerate}
    \item \textbf{Preliminaries}
    \begin{enumerate}
        \item Formal definition for dialogue evaluation.
        \item Formal definition for LLMs. How to utilize them to do the dialogue evaluation. In our paper, we will talk about logits method, generation methods. And the pros and cons for them. 
        \item Formal definition for Lora or other parameter efficient fine-tuning (PEFT) methods. 
        \item Different in-context example selection methods.
    \end{enumerate}
    \item \textbf{Experiment setup}
    \begin{enumerate}
        \item Data setup, one is open dataset (USS), the other one is Alexa internal dataset.
        \item LLMs setup, how many LLMs we used and size for them.
        \item In-context example selection methods setup.
        \item Supervised fine-tuning setup.
    \end{enumerate}
    \item \textbf{Experiment results and analysis}
    \begin{enumerate}
        \item \textbf{Larger model helps zero-shot dialogue evaluation}. Here we will use one table to clarify the results, or use one \textbf{figure}, [Scatter plot. x axis is the model size, y axis is the selected one metric, such as spearman correlation or pearson correlation.]
        \item \textbf{Instruction-tuning helps zero-shot dialogue evaluation}. Here we try to clarify this by utilizing one \textbf{table}, which compared the performance of some base model (Llama), and its instruct fine-tuning version of them (Alpaca). 
        \item \textbf{In-context examples enhance the performance of dialogue evaluation}. Here we will use a large table which focus on one model, but with few-shots settings including (random, bm25, bert) selected methods. We can conclude from the table that in-context example is useful.
        \item \textbf{How supervised fine-tuning influence the prediction results.} There will be large improvement compared to the original model after supervised fine-tuning.
        \item \textbf{Chain-of-thoughts for generation score and reasons}. In this part, we will talk about the performance of different chain-of-thoughts templates, first score then reasons and first analysis then score. We will find the second one is better in the one-shot settings. We utilize one example to let LLMs to generate output which follows the data structure we required. 
    \end{enumerate}
    \item \textbf{Related work}
    
    \item \textbf{Conclusion}
\end{enumerate}

==> tex/prompts.tex <==
\section{Prompts}
In this section, we elaborate on the prompts and instructions we used in the logits-based and generation-based evaluation methods. 
\subsection{Prompts for logits method} \label{subsec:prompts1}
The prompts we used in the logits method are formulated in the following manner:
\vspace*{-3mm}
\begin{tcolorbox}[width=\columnwidth,colback=white]
    \small
    \textbf{Instruction:}
    Could you please evaluate the subsequent dialogue by assigning a score from the given set [1,2,3,4,5]? A score of 1 implies dissatisfaction, while a 5 signifies high satisfaction.
\end{tcolorbox}

\subsection{Prompts for generation method}
\noindent \textbf{Rating-first}
In this section, we outline the prompts utilized in the Rating-First generation method. This process begins with an instruction that directs the Large Language Models (LLMs) to provide both reasons and ratings for a given dialogue. To enhance the LLMs' comprehension, we also supply evaluation criteria standards. Finally, we detail the evaluation steps necessary to complete the entire procedure for dialogue evaluation. The prompt is shown as follows:
\vspace*{-3mm}
\begin{tcolorbox}[width=\columnwidth,colback=white]
    \small{
    \textbf{Instruction}: Could you please evaluate 
    the subsequent dialogue, providing a score 
    from the set [1,2,3,4,5], and give an explanation 
    for choosing that score?\\
        \textbf{To help you better evaluate, here is the evaluation Criteria:}\\
        A score of 1 means very dissatisfied, where the user repeatedly has to stop or cancel bad responses and repeat their request again;\\
        A score of 2 means dissatisfied, where None of the user goals are achieved,the user expresses negative feedback,steps towards a user goal succeeds but the goal fails;\\
        A score of 3 means normal, where At least one of a user goals succeed, and no negative feedback\\
        A score of 4 means satisfied, where the majority of turns succeeded or moved the user closer to their goal\\
        A score of 5 means very satisfied, all turns either succeeded or moved the user closer to their goal(s), and the user\\ expressed no dissatisfaction, and goal was achieved without unnecessary steps\\
        \textbf{Steps to conduct the evaluation are:}\\
        1.Read the dialog, and the response carefully\\
        2.Rate the response on a scale of 1-5 for satisfaction level from user, according to the criteria above\\
        3.Provide a brief explanation for your rating, referring to specific aspects of the response and the dialog.\\}
\end{tcolorbox}

\noindent \textbf{Analysis-first}
In this section, we describe the prompts used in the Analysis-First generation method. Similar to the Rating-First approach, we begin by providing instructions for the LLMs to carry out dialogue evaluation. We then present specific aspects for the LLMs to analyze. To facilitate better understanding, we also supply the evaluation criteria. Finally, we detail the specific steps for the LLMs to follow.
\vspace*{-3mm}
\begin{tcolorbox}[width=\columnwidth,colback=white]
    \small{
    \textbf{Instruction}: Could you please evaluate the subsequent dialogue overall quality, 
    first analysis the dialogue from the following aspects:\\
    1.User goal. \\
    2.User feedback.\\
    3.System response.\\ 
    4.System feedback. \\
    Based the above analysis provide a user satisfactory score from the set [1,2,3,4,5]\\
        \textbf{To help you better evaluate, here is the evaluation Criteria:}\\
        A score of 1 means very dissatisfied, where the user repeatedly has to stop or cancel bad responses and repeat their request again;\\
        A score of 2 means dissatisfied, where None of the user goals are achieved,the user expresses negative feedback,steps towards a user goal succeeds but the goal fails;\\
        A score of 3 means normal, where At least one of a user goals succeed, and no negative feedback\\
        A score of 4 means satisfied, where the majority of turns succeeded or moved the user closer to their goal\\
        A score of 5 means very satisfied, all turns either succeeded or moved the user closer to their goal(s), and the user expressed no dissatisfaction, and goal was achieved without unnecessary steps\\
        \textbf{Steps to conduct the evaluation are:}\\
        1.Read the dialog, and the response carefully\\
        2.Give some brief analysis from the aspects mentioned before\\
        3.Rate the response on a scale of 1-5 for satisfaction level from user, according to the criteria above and the analysis.}
\end{tcolorbox}
\label{sec: prompts}
